Quantum integrable systems. Quantitative methods in biology

Quantum integrable systems have very strong mathematical properties that allow an exact description of their energetic spectrum. From the Bethe equations, I formulate the Baxter "T-Q" relation, that is the starting point of two complementary approaches based on nonlinear integral equations. The first one is known as thermodynamic Bethe ansatz, the second one as Kl\"umper-Batchelor-Pearce-Destri- de Vega. I show the steps toward the derivation of the equations for some of the models concerned. I study the infrared and ultraviolet limits and discuss the numerical approach. Higher rank integrals of motion can be obtained, so gaining some control on the eigenvectors. After, I discuss the Hubbard model in relation to the N = 4 supersymmetric gauge theory. The Hubbard model describes hopping electrons on a lattice. In the second part, I present an evolutionary model based on Turing machines. The goal is to describe aspects of the real biological evolution, or Darwinism, by letting evolve populations of algorithms. Particularly, with this model one can study the mutual transformation of coding/non coding parts in a genome or the presence of an error threshold. The assembly of oligomeric proteins is an important phenomenon which interests the majority of proteins in a cell. I participated to the creation of the project "Gemini" which has for purpose the investigation of the structural data of the interfaces of such proteins. The objective is to differentiate the role of amino acids and determine the presence of patterns characterizing certain geometries.

==> dati_I3_11cft.tex <==
I_3\text{ (CFT)}
0.0061979
4.2561979
19.131198
52.052045
22.560351
110.13688
55.125517
200.49775
112.78147
69.265146
35.980431


==> dati_I3_11tba.tex <==
    I_3\text{ (TBA)}
    0.0061979
    4.2561979
    19.131197
    52.052042
    22.560348
    110.13687
    55.125511
    200.49773
    112.78146
    69.265138
    35.980428


==> dati_I3_12cft.tex <==
I_3\text{ (CFT)}
-0.0063021
1.3686979
10.243698
33.732663
10.804733
78.939940
33.642011
16.699143
152.96762
78.030007
41.633949
43.143217


==> dati_I3_12tba.tex <==
    I_3\text{ (TBA)}
   -0.0063020
    1.3686970
    10.243694
    33.732653
    10.804732
    78.939920
    33.642008
    16.699141
    152.96759
    78.029998
    41.633947
    43.143213


==> dati_I5_11cft.tex <==
I_5\text{ (CFT)}
-0.0028301
8.1731074
104.14545
556.20159
108.29650
1943.8246
551.34946
5280.2710
1919.0972
636.39114
209.28433


==> dati_I5_11tba.tex <==
    I_5\text{ (TBA)}
   -0.0028301
    8.1731074
    104.14545
    556.20155
    108.29648
    1943.8244
    551.34937
    5280.2705
    1919.0969
    636.39101
    209.28430


==> dati_I5_12cft.tex <==
I_5\text{ (CFT)}
0.0026543
1.3062480
37.203592
271.05745
34.613169
1117.9764
255.64791
64.926784
3367.1124
1071.0704
283.29346
365.24996


==> dati_I5_12tba.tex <==
    I_5\text{ (TBA)}
    0.0026543
    1.3062466
    37.203567
    271.05732
    34.613163
    1117.9759
    255.64786
    64.926773
    3367.1113
    1071.0702
    283.29343
    365.24990

